Structural generalization in COGS: Supertagging is (almost) all you need

In many Natural Language Processing applications, neural networks have been found to fail to generalize on out-of-distribution examples. In particular, several recent semantic parsing datasets have put forward important limitations of neural networks in cases where compositional generalization is required. In this work, we extend a neural graph-based semantic parsing framework in several ways to alleviate this issue. Notably, we propose: (1) the introduction of a supertagging step with valency constraints, expressed as an integer linear program; (2) a reduction of the graph prediction problem to the maximum matching problem; (3) the design of an incremental early-stopping training strategy to prevent overfitting. Experimentally, our approach significantly improves results on examples that require structural generalization in the COGS dataset, a known challenging benchmark for compositional generalization. Overall, our results confirm that structural constraints are important for generalization in semantic parsing.

==> figures/cfq-transform.tex <==
\begin{figure}
    \centering
    \input{figures/cfq-tikz}
    \caption{
        \label{fig:cfq-transform}
        \textbf{(top)} The original semantic representation of the sentence "\emph{Did M1 star M0 's editor 's spouse}" in the CFQ dataset.
        \textbf{(bottom)} Our corresponding graph representation. We indicate node labels in black and arc labels in red.
    }
\end{figure}

==> sections/11-details.tex <==
\section{Training details}
\label{sec:details}

\paragraph{COGS development set.}
COGS only possesses an in-distribution development set and the accuracy of most parser on this set usually reaches 100\% quickly.
Previous work by \citet{conklin-etal-2021-meta} highlighted that not having a development set representative of the generalization set made model selection difficult and hard to reproduce.
As such, they proposed to sample a small subset of the generalization set that will be used as a development set for this purpose.
Similarly to this work and \citet{jambor-bahdanau-2022-lagr}, we sample a subset of 1000 sentences from the generalization set that we use as our development set.

\paragraph{Output fine-tuning.}
As presented in appendix \ref{sec:neural}, our model has an embedding and a bi-LSTM layers that produce a contextual representation for each word.
This representation is then used independently by each output layer to produce one of our four weight matrices.
To ensure that each of these layers is properly optimized, we fine-tune these layers after training.
This is done by freezing the every layer in the model except the output layer that we want to fine-tune.

==> sections/12-proof.tex <==
\section{Proof}
\label{app:proof}

We prove Theorem~\ref{th:supertagging} by reducing 3-dimensional matching to supertagging with companionship principle.

The 3-dimensional matching problem is defined as follows.
Let $A = \{a(1), ..., a(m)\}$, $B = \{b(1), ..., b(m)\}$ and $C = \{c(1), ..., c(m)\}$ be  3 sets of $m$ elements and $D \subseteq A \times B \times C$.
A subset $D' \subseteq D$ is a 3-dimensional matching if and only if, for any two distinct triples $(a, b, c) \in D'$ and $(a', b', c') \in D'$, the following three conditions hold:
\begin{itemize}
    \item $a \neq a'$,
    \item and $b \neq b'$,
    \item and $c \neq c'$.
\end{itemize}
The following decision problem is known to be NP-hard \cite{Karp1972}: given A, B, C and D, is there 3-dimensional matching $D' \subseteq D$ with $|D'| = m$?

We reduces this problem to supertagging with companionship constraint as follows.
We construct an instance of the problem with $3m$ concepts defined as $a(1), ..., a(m), b(1), ..., b(m), c(1), ..., c(m)$.
We construct the set of supertags $S$ as follows, where their associated weight is $0$ except when stated otherwise:
\begin{itemize}
    \item For each triple $(a, b, c) \in D$, we add a supertag $\llbracket (b, -), (c, -) \rrbracket$ with weight 1 if and only if it is predicted for concept $a$;
    \item For each $b \in B$, we add a supertag $\llbracket (b, +) \rrbracket$ with weight 1 if and only if it is predicted for concept $b$;
    \item For each $c \in C$, we add a supertag $\llbracket (c, +) \rrbracket$ with weight 1 if and only if it is predicted for concept $c$.
\end{itemize}
Then, if the solution of maximum supertagging with companionship constraint has a weight equal to $3m$, there exists a solution for the 3-dimensional matching decision problem.
This solution is given by the supertags associated with concepts $a(1), ..., a(m)$.

==> sections/13-extra.tex <==
\section{Extra results}
\label{sec:extra}

This section contains extra experimental results.
%Table~\ref{table:cogs-hinge} contains results using hinge losses instead of NLL losses.
Table~\ref{table:cogs-results2} contains results using a standard graph-based decoder that forces the semantic graph to be connected using the Maximum Spanning Connected Subgraph (MSCG) algorithm \cite{flanigan-etal-2014-discriminative}.
Finally, Figure~\ref{fig:valency-fail} shows an example where suppertaging fails if the companionship principle is not enforced.

%\input{tables/cogs-hinge}
\input{tables/cogs2}



==> tables/cfq.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{@{}l@{\hskip 0.25in}c@{\hskip 0.25in}c@{\hskip 0.25in}c@{\hskip 0.25in}c@{}}
\toprule
& Mean MCD & MCD1 & MCD2 & MCD3  \\
\midrule
\multicolumn{5}{@{}l@{}}{\textbf{Seq2seq approaches}} \\
\midrule
\citet{keysers2020measuring} 
& 18.9 & 37.4 & 8.1 & 11.3 \\
\citet{furrer-cfq}
& 42.1 & 61.6 & 31.3 & 33.3 \\
\citet{herzig-cfq}
& 22.6 & - & - & - \\
\midrule
\multicolumn{5}{@{}l@{}}{\textbf{Compositional approaches}} \\
\midrule
LaGR \cite{jambor-bahdanau-2022-lagr}
& 39.5 & 62.8 & 30.3 & 25.4 \\
HPD \cite{guo-cfq}
& 69.0 & 79.6 & 59.6 & 67.8 \\
\quad Without hierachical decoding
& 12.6 & 21.3 & 6.4 & 10.1 \\
LeAR \cite{liu-etal-2021-learning-algebraic}
& 90.9 & 91.7 & 89.2 & 91.7 \\
\quad Without Tree-LSTM
& 30.4 & 40.1 & 25.6 & 25.4 \\
\midrule
Our approach (best results)
& 65.7 & 81.7 & 61.3 & 54.1 \\
\quad Valency aware variant
& - & - & - & - \\
\quad Valency unaware variant
& 65.7 & 81.7 & 61.3 & 54.1 \\
\quad Without label sets
& 36.1 & 64.2 & 23.8 & 20.3 \\
\bottomrule
\end{tabular}
\caption{Accuracy on the CFQ dataset. We report the accuracy over each MCD split as well as the mean of these accuracies.}
\label{table:cfq-results}
\end{table*}

==> tables/cogs-hinge.tex <==
\begin{table*}[!t]
\small
\centering
\begin{tabular}{@{}l@{\hskip 0.05in}ccc@{\hskip 0.15in}c@{\hskip 0.15in}c@{}}
\toprule
& \multicolumn{3}{c@{\hskip 0.15in}}{Structural} & Lexical & Overall  \\
\cmidrule(r{0.15in}){2-4}
& Obj to Subj PP & PP recursion & CP recursion & & \\

%\midrule
%\multicolumn{6}{@{}l@{}}{\textbf{Baseline with MSCG inference}} \\
%\midrule
%Hinge loss
%& 13.8 & 0 & 0 & 97.5 & 84.3 \\
%& 0 & 0 & 0 & 0 & 0 \\
%\quad w/o auxiliary obj.
%& 11.0 & 0 & 0 & 96.4 & 83.2 \\
%& 0 & 0 & 0 & 0 & 0 \\

\midrule
\multicolumn{6}{@{}l@{}}{\textbf{Graph-based decoder baseline}} \\
\midrule
Hinge loss
%& 11.9 & 0 & 0 & 97.4 & 84.1 \\
& 0 & 0 & 0 & 0 & 0 \\
\quad w/o auxiliary obj.
%& 9.3 & 0 & 0 & 96.4 & 83.1 \\
& 0 & 0 & 0 & 0 & 0 \\

\midrule
\multicolumn{6}{@{}l@{}}{\textbf{Our approach}} \\
\midrule
Hinge loss 
%& 48.1 & \textbf{100} & \textbf{100} & 98.3 & 96.1 \\
& 0 & 0 & 0 & 0 & 0 \\

\bottomrule
\end{tabular}
\caption{Exact match accuracy using hinge losses instead of NLL losses.}
\label{table:cogs-hinge}
\end{table*}

==> tables/cogs2.tex <==
\begin{table*}[!t]
\small
\centering
\begin{tabular}{@{}l@{\hskip 0.05in}ccc@{\hskip 0.15in}c@{\hskip 0.15in}c@{}}
\toprule
& \multicolumn{3}{c@{\hskip 0.15in}}{Structural} & Lexical & Overall  \\
\cmidrule(r{0.15in}){2-4}
& Obj to Subj PP & PP recursion & CP recursion & & \\

\midrule
\multicolumn{6}{@{}l@{}}{\textbf{Baseline with MSCG inference}} \\
\midrule
Early stopping
& 13.7 & 0 & 0 & 97.5 & 84.3 \\
\quad w/o early stopping
& 15.8 & 0 & 0 & 97.5 & 84.4 \\
\quad w/o early stopping + w/o auxiliary obj.
& 11.7 & 0 & 0 & 97.5 & 84.2 \\
\bottomrule
\end{tabular}
\caption{Exact match accuracy using the MSCG algorithm in a graph-based semantic parser.}
\label{table:cogs-results2}
\end{table*}
